The Salvetti Complex and the Little Cubes

We study how the combinatorial structure of the Salvetti complexes of the braid arrangements are related to homotopy theoretic properties of iterated loop spaces. We prove the skeletal filtrations on the Salvetti complexes of the braid arrangements give rise to the cobar-type Eilenberg-Moore spectral sequence converging to the homology of $\Omega^2\Sigma^2 X$. We also construct a new spectral sequence that computes the homology of $\Omega^{\ell}\Sigma^{\ell} X$ for $\ell>2$ by using a higher order analogue of the Salvetti complex. The $E^1$-term of the spectral sequence is described in terms of the homology of $X$. The spectral sequence is different from known spectral sequences that compute the homology of iterated loop spaces, such as the Eilenberg-Moore spectral sequence and the spectral sequence studied by Ahearn and Kuhn.

==> arrangements.tex <==
\section{Recollections on arrangements of hyperplanes}
\label{Arrangements}

Let us recall basic properties of arrangement of hyperplanes and fix
notations and terminologies.

Let $\mathcal{H} = \{M_j\}_{j\in J}$ be a collection of hyperplanes in
$\R^n$. We assume that $\mathcal{H}$ is central, i.e.\ 
$\cap_{j\in J} M_j \neq \emptyset$. $\mathcal{H}$ defines a
stratification of $\R^n$.
\begin{eqnarray*}
 M^0 & = & \R^n-\bigcup_{j\in J} M_j \\
 M^1 & = & \bigcup_{j\in J} \left(M_j- \bigcup_{k\neq j} M_j\cap
			     M_k\right) \\
 & \vdots & \\
 M^{|J|} & = & \bigcap_{j\in J} M_j \\
 \R^n & = & M^0\cup M^1\cup \cdots \cup M^{|J|}
\end{eqnarray*}

The connected components of each stratum are called facets and a facet
in the top stratum is called a chamber. For each facet $F$, the affine
hull of $F$ is denoted by $|F|$.

We use the following notations:
\begin{eqnarray*}
 \mathcal{F}(\mathcal{H}) & = & \{\text{facets of }\mathcal{H}\} \\
 \mathcal{F}^i(\mathcal{H}) & = & \{F\in\mathcal{F}(\mathcal{H}) \mid
  \codim F = i\}
\end{eqnarray*}

We need an ordering in $\mathcal{F}(\mathcal{H})$. Although a popular
way to define an ordering is by the ``reverse inclusion'', Salvetti
defines as follows
\[
 F\ge F' \Longleftrightarrow \overline{F} \supset F'.
\]

Given an arrangement $\mathcal{H}$ in $\R^n$ and a subset $F \subset
\R^n$, there are two ways to restrict $\mathcal{H}$ to obtain a smaller
arrangement.

\begin{definition}
 For a hyperplane arrangment $\mathcal{H}$ in $\R^n$ and a subset
 $F \in \R^n$, define
 \begin{eqnarray*}
  \mathcal{H}_{\supset F} & = & \{H \in \mathcal{H} \mid H\supset F\}, \\
  \mathcal{H}|_{F} & = & \{H\cap F \mid H \in \mathcal{H}\}.
 \end{eqnarray*}
\end{definition}

Salvetti studies the complement of the complexification of a real
arrangement.

\begin{definition}
 For a hyperplane
 \[
 M = \{\bm{x}\in\R^n \mid \langle\bm{a},\bm{x}\rangle = c\}
 \]
 its complexification is denoted by
 \[
 M^{\C} = \{\bm{z}\in\C^n \mid \langle\bm{a},\bm{z}\rangle = c\}.
 \]
 For a real arrangement $\mathcal{H}$, its complexification is denoted
 by
 \[
  \mathcal{H}^{\C} = \{H^{\C} \mid H\in \mathcal{H}\}.
 \]
\end{definition}


==> cells_in_higher_Salvetti.tex <==
\subsection{Cellular Structures on Higher Order Salvetti Complexes}
\label{cells_in_higher_Salvetti}


